Small- and Large-Scale Galactic Conformity in SDSS DR7

Galactic conformity is the phenomenon whereby galaxy properties exhibit excess correlations across distance than that expected if these properties only depended on halo mass. We perform a comprehensive study of conformity at low redshift using a galaxy group catalogue from the SDSS DR7 spectroscopic sample. We study correlations both between central galaxies and their satellites (1-halo), and between central galaxies in separate haloes (2-halo). We use the quenched fractions and the marked correlation function (MCF), to probe for conformity in three galaxy properties, $(g-r)$ colour, specific star formation rate (sSFR), and morphology. We assess the statistical significance of conformity signals with a suite of mock galaxy catalogues that have no built-in conformity, but contain the same group-finding and mass assignment errors as the real data. In the case of 1-halo conformity, quenched fractions show strong signals at all group masses. However, these signals are equally strong in mock catalogues, indicating that the conformity signal is spurious and likely entirely caused by group-finding systematics, calling into question previous claims of 1-halo conformity detection. The MCF reveals a significant detection of radial segregation within massive groups, but no evidence of conformity. In the case of 2-halo conformity, quenched fractions show no significant evidence of conformity in colour or sSFR once compared with mock catalogues, but a clear signal using morphology. In contrast, the MCF reveals a small, yet highly significant signal for all three properties in low mass groups and scales of $0.8-4\ h^{-1}\textrm{Mpc}$, possibly representing the first robust detection of 2-halo conformity.

==> hyperlink-year-only-natbib-patch.tex <==
% found on https://tex.stackexchange.com/questions/23227/how-to-hyperlink-only-the-year-part-when-using-natbib-and-hyperref

\RequirePackage{hyperref}
\RequirePackage{natbib}
\RequirePackage{etoolbox}

\makeatletter

% Patch case where name and year are separated by aysep
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\makeatother


==> submission_notes.tex <==
Small- and Large-Scale Galactic Conformity in SDSS DR7

Victor Calderon, Andreas Berlind, Manodeep Sinha

Galactic conformity is the phenomenon whereby galaxy properties exhibit
excess correlations across distance than that expected if these properties
only depended on halo mass. We perform a comprehensive study of conformity
at low redshift using a galaxy group catalogue from the SDSS DR7
spectroscopic sample. We study correlations both between central galaxies
and their satellites (1-halo), and between central galaxies in separate haloes
(2-halo). We use the quenched fractions and the marked correlation function
(MCF), to probe for conformity in three galaxy properties, $(g-r)$ colour,
specific star formation rate (sSFR), and morphology. We assess the
statistical significance of conformity signals with a suite of mock galaxy
catalogues that have no built-in conformity, but contain the same
group-finding and mass assignment errors as the real data. In the case of
1-halo conformity, quenched fractions show strong signals at all group
masses. However, these signals are equally strong in mock catalogues,
indicating that the conformity signal is spurious and likely entirely
caused by group-finding systematics, calling into question previous claims
of 1-halo conformity detection. The MCF reveals a significant detection
of radial segregation within massive groups, but no evidence of conformity.
In the case of 2-halo conformity, quenched fractions show no significant
evidence of conformity in colour or sSFR once compared with mock catalogues,
but a clear signal using morphology. In contrast, the MCF reveals a small,
yet highly significant signal for all three properties in low mass groups
and scales of $0.8-4\ h^{-1}\textrm{Mpc}$, possibly representing the first
robust detection of 2-halo conformity.

16 pages, 5 figures, accepted to MNRAS

